Safety Embedded Adaptive Control Using Barrier States

In this work, we explore the application of barrier states (BaS) in the realm of safe nonlinear adaptive control. Our proposed framework derives barrier states for systems with parametric uncertainty, which are augmented into the uncertain dynamical model. We employ an adaptive nonlinear control strategy based on a control Lyapunov functions approach to design a stabilizing controller for the augmented system. The developed theory shows that the controller ensures safe control actions for the original system while meeting specified performance objectives. We validate the effectiveness of our approach through simulations on diverse systems, including a planar quadrotor subject to unknown drag forces and an adaptive cruise control system, for which we provide comparisons with existing methodologies.

==> commands.tex <==
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{comment}
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{enumerate}
% \usepackage{subfigure}

% \usepackage{subcaption}
% \usepackage[caption=false]{subfig}

\usepackage{soul}
\usepackage{xcolor}

\usepackage{hyperref}
\hypersetup{
    % colorlinks=true,
    linkcolor=black,
    filecolor=black,      
    urlcolor=black,
}



\usepackage[style=ieee]{biblatex}
  
\AtBeginBibliography{\scriptsize}  %\small %\footnotesize %\scriptsize
\addbibresource{IEEEfull.bib}

% \usepackage[numbers]{natbib}
%\def\bibfont{\footnotesize}  %\small %\footnotesize %\scriptsize


\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\theoremstyle{definition}
\newtheorem{definition}{Definition}%[section]
\renewcommand{\qedsymbol}{$\blacksquare$}
\renewcommand{\figureautorefname}{Fig.}
\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Subsection}
\newcommand{\definitionautorefname}{Definition}
\newcommand{\propositionautorefname}{Proposition}
\newcommand{\lemmaautorefname}{Lemma}
\newtheorem{remark}{Remark}
\newcommand{\remarkautorefname}{Remark}
\newcommand{\corollaryautorefname}{Corollary}
\newtheorem{assumption}{Assumption}
\newcommand{\assumptionautorefname}{Assumption}
\newtheorem{problem}{Problem}

\newcommand{\problemautorefname}{Problem}


\newcommand{\hassan}[1]{\textcolor{blue}{\textbf{Hassan:} #1}}
\newcommand{\john}[1]{\textcolor{green}{\textbf{John:} #1}}
\newcommand{\maitham}[1]{\textcolor{red}{\textbf{Maitham:} #1}}
